On the Bottleneck of Graph Neural Networks and its Practical Implications

Since the proposal of the graph neural network (GNN) by Gori et al. (2005) and Scarselli et al. (2008), one of the major problems in training GNNs was their struggle to propagate information between distant nodes in the graph. We propose a new explanation for this problem: GNNs are susceptible to a bottleneck when aggregating messages across a long path. This bottleneck causes the over-squashing of exponentially growing information into fixed-size vectors. As a result, GNNs fail to propagate messages originating from distant nodes and perform poorly when the prediction task depends on long-range interaction. In this paper, we highlight the inherent problem of over-squashing in GNNs: we demonstrate that the bottleneck hinders popular GNNs from fitting long-range signals in the training data; we further show that GNNs that absorb incoming edges equally, such as GCN and GIN, are more susceptible to over-squashing than GAT and GGNN; finally, we show that prior work, which extensively tuned GNN models of long-range problems, suffers from over-squashing, and that breaking the bottleneck improves their state-of-the-art results without any tuning or additional weights. Our code is available at https://github.com/tech-srl/bottleneck/ .

==> 04-breaking.tex <==
\section{Breaking the Bottleneck}\label{sec:breaking}

To overcome the bottleneck, we wish to allow a node to interact directly with nodes that reside beyond its immediate neighbors. The information propagated from these distant nodes might have been lost or noised in the bottleneck. However, we do \emph{not} wish to connect every node to every other node across all message propagation steps, because this ignores the topology of the graph and increases the computational complexity from $O\left(|\mathcal{E}| \right)$ to $O\left(|\mathcal{V}|^2 \right)$ across all layers.

To break the bottleneck, we propose to add a single \emph{clique layer} on top of a GNN stack containing $K$ layers.
A clique layer is a GNN layer where every node is connected to any other node:
\begin{equation}
    \mathbf{h}_v^{\left(clique\right)}=f_{clique}\left(
    \mathbf{h}_v^{\left(K\right)}, 
    \{\mathbf{h}_u^{\left(K\right)}\mid u\in \mathcal{V}\}
    ; \theta_{clique}\right)
    \label{eq:clique}
\end{equation}
Where $f_{clique}$ can either be the same function as in the rest of the layers $f_{1..K}$,
or a different interaction function between a node and a set of nodes. Note that \Cref{eq:clique} is very similar to \Cref{eq:layer}, except that in \Cref{eq:layer} the interaction is only with the neighbors of $v$ (i.e., $\mathcal{N}_v$),
and in \Cref{eq:clique} the interaction is with all the nodes in the graph ($\mathcal{V}$) \uri{candidate for removal}.

Clique layers allow interactions between topology-aware node representations of the $K$-'th layer, even if they are distant, while still allowing a GNN to leverage the graph topology using the original $K$ layers.
Additionally, clique layers free the GNN from having to squash all the information flowing into a node into a fixed-length vector, regardless of the graph size.
For example, if the node under prediction in \Cref{fig:cloud} could interact with the node marked with ``C'' directly, after both have counted the number of their blue neighbors, we could predict the label of the node in question without squashing the information from the entire graph into a fixed-length vector.




==> broader_impact.tex <==
\section*{Broader Impact}
This work discusses a general limitation of graph neural networks. This work thus has no direct ethical or societal consequences.

==> combinatorial-additional.tex <==
\section{Combinatorial Analysis}
\label{sec:stats-additional}
We analyize the  combinatorial upper bound for the maximal depth that a GNN can perfectly fit (learn to 100\% training accuracy) given its hidden vector size $d$. 
We denote the arity of such a tree by $m$ ($=$$2$ in our experiments);
the counting base as $b$$=$$2$; %
the number of bits in a floating-point variable as $f$$=$$32$; %
and the hidden dimension of the GNN, i.e., the size of a node vector 
$\mathbf{h}_v^{\left(k\right)}$, as $d$.

A full tree of arity $m$ has $m^{depth}$ leaves.
As described in \Cref{subsec:synthetic}, given an arrangement of blue neighbors, all possible permutations of the labels \{A, B, C, ...\} are valid. Thus, the number of leaf label assignments is $\left(m^{depth}\right)!$.
Right before interacting with the target node and predicting the label, a single vector of size $d$ must encapsulate the information flowing from all leaves (\Cref{eq:gcn,eq:gin}).\footnote{The analysis holds for GCN and GIN. Architectures that use the representation of the recipient node to aggregate messages, like GAT, need to compress the information from only \emph{half} of the leaves in a single vector. This increases the final upper bounds of $depth$ by up to 1 and demonstrated empirically in \Cref{subsec:synthetic}.}
Such a vector contains $d$ floating-point elements, each of them is stored as $f$ bits. Overall, the number of possible cases that this vector can distinguish between is $b^{f\cdot d}$. The number of possible cases that the vector can distinguish between must be greater than the number of different examples this vector may encounter in the training data. 

 \Cref{eq:dim-depth};
considering binary trees ($m$$=$$2$), and floating-point values of $f$$=$$32$ binary ($b$$=$$2$) bits, we get \Cref{eq:dim-depth-concrete}:
\newline
\noindent\begin{minipage}[t]{.5\linewidth}
\begin{equation}
	\left(m^{depth}\right)!  < b^{f\cdot d}
	\label{eq:dim-depth2}
\end{equation}
\end{minipage}
\noindent\begin{minipage}[t]{.5\linewidth}
\begin{equation}
	\left(2^{depth}\right)!  < 2^{32\cdot d}
	\label{eq:dim-depth-concrete2}
\end{equation}
\end{minipage}

Now, we can fix either $d$ or $depth$ and solve for the other. For example, in \Cref{fig:dim-depth} we fixed different values of $d$ and found the maximal $depth\in \mathbb{N}$ that satisfies \Cref{eq:dim-depth-concrete}, to get the combinatorial max $depth$ for each value of $d$.

==> dim-depth-table.tex <==

\begin{table*}[t]
    \centering
    \footnotesize
    \begin{tabular}{lcccccccc}
        \toprule
          & $d$$=$4 & $d$$=$8 & $d$$=$16 & $d$$=$32 & $d$$=$64 & $d$$=$128 & $d$$=$256 & $d$$=$512 \\
         \midrule
		combinatorial max $depth$: & 5 & 5 & 6 & 7 & 8 & 9 & 9 & 10 \\
		empirical max $depth$: & & & & 3 & & & & \\
        \bottomrule
    \end{tabular}
    \caption{The combinatorial upper bound of $depth$ given $d$, the model dimension. The empirical max $depth$ is the maximal depth that a GCN successfully fits to 100\% training accuracy.}
    \label{tab:dim-depth}
\end{table*} 

==> qm_results1.tex <==

\begin{table*}[t]
    \centering
    \footnotesize
    \begin{tabu}{lrrrrrrrr}
        \toprule
        \rowfont{\footnotesize}
        	& \multicolumn{2}{c}{GNN-MLP0} & & \multicolumn{2}{c}{R-GAT} & &\multicolumn{2}{c}{GNN-FiLM }\\         
\cmidrule{2-3} \cmidrule{5-6} \cmidrule{8-9}
\rowfont{\footnotesize}
        \scriptsize{Property} & \multicolumn{1}{c}{base$^{\dagger}$} & \multicolumn{1}{c}{$+$FA} & & \multicolumn{1}{c}{base$^{\dagger}$}& \multicolumn{1}{c}{$+$FA} & & \multicolumn{1}{c}{base$^{\dagger}$} & \multicolumn{1}{c}{$+$FA} \\
        \midrule
        \footnotesize{mu}  & 2.36$\pm$0.04 & {\textbf{2.19}}$\pm$0.04 & & \textbf{2.68}$\pm$0.06  & 2.73$\pm$0.07 &  & 2.38$\pm$0.13 & \textbf{2.26}$\pm$0.06 \\
        \footnotesize{alpha}  & 4.27$\pm$0.36 &  {\textbf{1.92}}$\pm$0.06 &   & 4.65$\pm$0.44 & \textbf{2.32}$\pm$0.16 &  & 3.75$\pm$0.11 & \textbf{1.93}$\pm$0.08\\
        \footnotesize{HOMO}  & 1.25$\pm$0.04 & \textbf{1.19}$\pm$0.04 &   &  1.48$\pm$0.03 & \textbf{1.43}$\pm$0.02&  & 1.22$\pm$0.07 & {\textbf{1.11}}$\pm$0.01 \\
        \footnotesize{LUMO}  & 1.35$\pm$0.04 & {\textbf{1.20}}$\pm$0.05 &  & 1.53$\pm$0.07 & \textbf{1.41}$\pm$0.03&  & 1.30$\pm$0.05 & \textbf{1.21}$\pm$0.05 \\
        \footnotesize{gap}  & 2.04$\pm$0.05 & \textbf{1.82}$\pm$0.05 &  &  2.31$\pm$0.06 & \textbf{2.08}$\pm$0.05 &  & 1.96$\pm$0.06 & {\textbf{1.79}}$\pm$0.07 \\
        \footnotesize{R2}  & 14.86$\pm$1.62 & \textbf{12.40}$\pm$0.84 &  & 52.39 $\pm$42.5 & \textbf{15.76}$\pm$1.17 &  & 15.59$\pm$1.38 & {\textbf{11.89}}$\pm$0.73 \\
        \footnotesize{ZPVE}  & 12.00$\pm$1.66 & {\textbf{4.68}}$\pm$0.29 &  & 14.87$\pm$2.88 & \textbf{5.98}$\pm$0.43  &  & 11.00$\pm$0.74 & {\textbf{4.68}}$\pm$0.49 \\
        \footnotesize{U0}  & 5.55$\pm$0.38 & \textbf{1.71}$\pm$0.13 &  & 7.61$\pm$0.46 &\textbf{2.19}$\pm$0.25 &  & 5.43$\pm$0.96 & {\textbf{1.60}}$\pm$0.12 \\
        \footnotesize{U}  & 6.20$\pm$0.88 & {\textbf{1.72}}$\pm$0.12&  & 6.86$\pm$0.53 & \textbf{2.11}$\pm$0.10&  & 5.95$\pm$0.46 & \textbf{1.75}$\pm$0.08 \\
        \footnotesize{H}  & 5.96$\pm$0.45  & {\textbf{1.70}}$\pm$0.08 &  & 7.64$\pm$0.92 & \textbf{2.27}$\pm$0.29 &  & 5.59$\pm$0.57 & \textbf{1.93}$\pm$0.42 \\
        \footnotesize{G}  & 5.09$\pm$0.57 & {\textbf{1.53}}$\pm$0.15 &  & 6.54$\pm$0.36 & \textbf{2.07}$\pm$0.07 &  & 5.17$\pm$1.13 & \textbf{1.77}$\pm$0.05 \\
        \footnotesize{Cv}  & 3.38$\pm$0.20 & \textbf{1.69}$\pm$0.08 &  & 4.11$\pm$0.27 & \textbf{2.03}$\pm$0.14 &  & 3.46$\pm$0.21 & {\textbf{1.64}}$\pm$0.10 \\
        \footnotesize{Omega}  &  0.84$\pm$0.02 &  {\textbf{0.63}}$\pm$0.04 &  & 1.48$\pm$0.87 & \textbf{0.73}$\pm$0.04 &  & 0.98$\pm$0.06 & \textbf{0.69}$\pm$0.05 \\
        \midrule
        relative & \multicolumn{2}{c}{-40.33\%} & & \multicolumn{2}{c}{-44.58\%} & & \multicolumn{2}{c}{-39.53\%} \\
        \bottomrule
    \end{tabu}
    \caption{Average error rates and standard deviations on the QM9 targets. Best result for every property in every GNN type is highlighted in bold. %
    Results marked with ${\dagger}$ were previously reported by \citet{brockschmidt2019graph}.}
    \label{tab:qm-results}
\end{table*} 

==> varmisuse-results.tex <==


\begin{table*}[t]
    \centering
    \vspace{-2.5mm}
    \footnotesize
    \begin{tabular}{clrrrrr}
    \toprule
    & & \multicolumn{1}{c}{GGNN} & \multicolumn{1}{c}{R-GCN} & \multicolumn{1}{c}{R-GIN} & \multicolumn{1}{c}{GNN-MLP} &  \multicolumn{1}{c}{R-GAT} \\ %
    \midrule


	\multirow{2}{*}{SeenProj Test} & base  & 85.7$\pm$0.5 & 88.3$\pm$0.4 & 87.1$\pm$0.1 & 86.9$\pm$0.3 & 86.9$\pm$0.7 \\
	& $+$FA  & \textbf{86.3}$\pm$0.7 & \textbf{88.4}$\pm$0.7 & \textbf{87.5}$\pm$0.7 & \textbf{87.3}$\pm$0.2 & \textbf{87.9}$\pm$1.0\\
	\midrule
    \multirow{2}{*}{UnseenProj Test} & base & \textbf{79.3}$\pm$1.2 & 82.9$\pm$0.8 & 81.1$\pm$0.9 & \textbf{81.4}$\pm$0.7 & 81.2$\pm$0.9 \\
    	& $+$FA  & 79.1$\pm$1.1 & \textbf{83.8}$\pm$1.0 & \textbf{81.7}$\pm$1.2 & 81.2$\pm$0.5 & \textbf{82.0}$\pm$1.9 \\
    \bottomrule
    \end{tabular}
    \caption{
    Average accuracy and standard deviations on {\sc{VarMisuse}}. 
    }
    \label{tab:varmisuse-results-flat}
\end{table*} 
